Wandering Within a World: Online Contextualized Few-Shot Learning

We aim to bridge the gap between typical human and machine-learning environments by extending the standard framework of few-shot learning to an online, continual setting. In this setting, episodes do not have separate training and testing phases, and instead models are evaluated online while learning novel classes. As in the real world, where the presence of spatiotemporal context helps us retrieve learned skills in the past, our online few-shot learning setting also features an underlying context that changes throughout time. Object classes are correlated within a context and inferring the correct context can lead to better performance. Building upon this setting, we propose a new few-shot learning dataset based on large scale indoor imagery that mimics the visual experience of an agent wandering within a world. Furthermore, we convert popular few-shot learning approaches into online versions and we also propose a new contextual prototypical memory model that can make use of spatiotemporal contextual information from the recent past.

==> sections/impact.tex <==
% !TEX root = ../main.tex
\section*{Broader Impact}
\vspace{-0.1in}
Our work aims to bridge the gap between machine learning and human learning in terms of the
adaptibility at test time of recognizing novel objects. Potential applications include more
personalized assistive technology and general home robotics. For example, as the society ages, the
population needs additional caregiving at home, but this option is currently not available to
everyone. Having a robot that can cook and do laundry at home can greatly alleviate the burden to
many people. We also note that while our intention is good, just like all technologies, the
algorithm we develop can also bring disadvantages to certain groups, for example, people who cannot
afford products sold by companies that have put in their resources to commercialize the
technological advances made by us, and people or facilities that are targeted by autonomous
surveillance and weapons. Whether the potential impact is positive or negative is unclear to us and
we would like to leave it open to debate.

==> tables/table_datasets.tex <==
% !TEX root = ../main.tex
\begin{table}[t]
\vspace{-0.3in}
\begin{minipage}[t]{0.45\textwidth}
\begin{small}
\begin{center}
\caption{\small Comparison of past FSL and CL tasks vs. our online contextualized FSL}
\label{tab:benchmark}
\vspace{-0.1in}
\resizebox{!}{1.3cm}{% <------ Don't forget this %
\begin{tabular}{ccccccc}
\toprule
                                      % & \mc{2}{c|}{\bf Supervision Type}  & \mc{2}{c|}{\bf Continual}       & \mc{2}{c|}{\bf Output \& Context} &    \mc{2}{c}{\bf Context}       \\
\mr{2}{\tb{Tasks}}                    & \tb{Few}  & \tb{Semi-supv. } & \mr{2}{\tb{Cont'}} & \tb{Online} & \tb{Predict}& \tb{Soft Ctx.}  \\
                                      & \tb{Shot} & \tb{Supp. Set}   &                    & \tb{Eval.}  & \tb{New}    & \tb{Switch}     \\
\midrule                                                                                                                                                                       
Inc. Learning (IL)                    & \xm       & \xm              & \cm                & \hx         & \xm         & \xm             \\
Few-shot (FSL) \citep{matchingnet}     & \cm       & \xm              & \xm                & \xm         & \xm         & \xm             \\
Incremental FSL \citep{attnattractor}  & \cm       & \xm              & \hx                & \xm         & \xm         & \xm             \\
% Cls. Inc. FSL \cite{fscil}          & \cm       & \xm              & \cm                & \hx         & \xm         & \xm             \\
Semi-supv. FSL \citep{fewshotssl}      & \cm       & \cm              & \xm                & \xm         & \cm         & \xm             \\
% Continual Meta-Learning             & \mr{2}{\cm} & \mr{2}{\xm}    & \mr{2}{\cm}        & \mr{2}{\xm} & \mr{2}{\xm} & \mr{2}{\hx}     \\
% w/o Tasks \cite{moca}                 &                       &                      &                        &                  &                    &                                        \\
Online Mixture \citep{onlinemixture}   & \cm       & \xm              & \cm                & \xm         & \xm         & \hx                                    \\
Online Meta \citep{oml}                & \cm                   & \xm                  & \cm                    & \xm              & \xm                & \xm                                    \\
Continual FSL \citep{contfsl}          &\mr{2}{\cm}            &  \mr{2}{\xm}         & \mr{2}{\cm}            & \mr{2}{\xm}      & \mr{2}{\xm}        & \mr{2}{\xm}                            \\
 (Concurrent Work)                    &                       &                      &                        &                  &                    &                                        \\
\midrule                                                                                                                                                                                         
OC-FSL (Ours)      & \cm                   & \cm                  & \cm                    & \cm              & \cm                & \cm                                    \\
\bottomrule
\end{tabular}
}
\end{center}
\end{small}
\end{minipage}
\hfill
\begin{minipage}[t]{0.53\textwidth}
\begin{small}
\begin{center}
\caption{\small Common continual \& few-shot learning datasets vs. the new MP3D OC-FSL dataset}
\label{tab:dataset_stats}
\vspace{-0.1in}
\resizebox{!}{1.3cm}{% <------ Don't forget this %
\begin{tabular}{ccccccc}
\toprule
                              & {\bf Img.} & {\bf Sess.} & {\bf Cls.} & {\bf Content}                  \\
\midrule                                                                     
Permuted MNIST~\citep{mnist}   & 60K          & -           & -          & Hand written digits          \\
Omniglot~\citep{omniglot}      & 32.4K        & -           & 1.6K       & Hand written characters      \\
CIFAR-100~\citep{cifar}        & 50K          & -           & 100        & Common objects               \\
mini-ImageNet~\citep{matchingnet}& 50K        & -           & 100        & Common objects               \\
tiered-ImageNet~\citep{fewshotssl}& 779K      & -           & 608        & Common objects               \\
% ImageNet                      & 1.3M         & -           & 1K         & Common objects                  \\
OpenLORIS  \citep{openloris}   & 98K          & -           & 69         & Small table-top obj.         \\ 
CORe50  \citep{core50}         & 164.8K       & 11          & 50         & Hand-held obj.               \\
\midrule                                                                                                          
MP3D OC-FSL (Ours)            & 1.2K         & 6.9K        & 7.0K       & General indoor instances     \\
\bottomrule
\end{tabular}
}
\end{center}
\end{small}
\end{minipage}
\vspace{-0.2in}
\end{table}

